Learned D-AMP: Principled Neural Network based Compressive Image Recovery

Compressive image recovery is a challenging problem that requires fast and accurate algorithms. Recently, neural networks have been applied to this problem with promising results. By exploiting massively parallel GPU processing architectures and oodles of training data, they can run orders of magnitude faster than existing techniques. However, these methods are largely unprincipled black boxes that are difficult to train and often-times specific to a single measurement matrix. It was recently demonstrated that iterative sparse-signal-recovery algorithms can be "unrolled" to form interpretable deep networks. Taking inspiration from this work, we develop a novel neural network architecture that mimics the behavior of the denoising-based approximate message passing (D-AMP) algorithm. We call this new network Learned D-AMP (LDAMP). The LDAMP network is easy to train, can be applied to a variety of different measurement matrices, and comes with a state-evolution heuristic that accurately predicts its performance. Most importantly, it outperforms the state-of-the-art BM3D-AMP and NLR-CS algorithms in terms of both accuracy and run time. At high resolutions, and when used with sensing matrices that have fast implementations, LDAMP runs over $50\times$ faster than BM3D-AMP and hundreds of times faster than NLR-CS.

==> Learned D-AMP NIPS 2017_arxiv/Conclusions.tex <==
\section{Conclusions}
In this paper, we have developed, analyzed, and validated a novel neural network architecture that mimics the behavior of the powerful D-AMP signal recovery algorithm.
The LDAMP network is easy to train, can be applied to a variety of different measurement matrices, and comes with a state-evolution heuristic that accurately predicts its performance. Most importantly, LDAMP outperforms the state-of-the-art BM3D-AMP and NLR-CS algorithms in terms of both accuracy and run time.

LDAMP represents the latest example in a trend towards using training data (and lots of offline computations) to improve the performance of iterative algorithms.
The key idea behind this paper is that, rather than training a fairly arbitrary black box to learn to recover %sparse
signals, we can unroll a conventional iterative algorithm and treat the result as a NN, which produces a network with well-understood behavior, performance guarantees, and predictable shortcomings. It is our hope this paper highlights the benefits of this approach and encourages future research in this direction.

%\FloatBarrier

==> Learned D-AMP NIPS 2017_arxiv/Experiments.tex <==
\section{Experiments}\label{sec:expmt}
% In this section we describe how we implemented, trained, and tested LDAMP, LDVAMP, and LDIT.

% \subsection{Implementation}
% % \paragraph{Implementation}
% We implemented LDAMP and LDIT, using the DnCNN denoiser \cite{DnCNN}, with both TensorFlow and MatConvnet \cite{vedaldi15matconvnet}, a convolutional neural network toolbox for Matlab. % We plan to make both implementations publicly available.. 
% %We also implemented a Learned version of D-VAMP \cite{DVAMP} (LDVAMP).
% %With the measurement matrices used in this section, LDVAMP had performance nearly identical to that of LDAMP, and so for brevity we do not present results for LDVAMP.\footnote{For measurement matrices which are right rotationally invariant but not i.i.d.~ subgaussian the performance of LDVAMP should significantly excede that of LDAMP.}
% The MatConvnet implementation of DnCNN was provided by the its authors here \url{https://github.com/cszn/DnCNN}. The results reported in this section are for the MatConvnet version of the network.

% %At present, the python implementation uses a fixed denoiser at every layer whereas the MatConvnet implementation selects which denoiser to use at each layer based on an estimate of the standard deviation of the effective noise.

\paragraph{Datasets}
Training images were pulled from Berkeley's BSD-500 dataset \cite{BSDDataset}. 
From this dataset, we used 400 images for training, 50 for validation, and 50 for testing. %training images, 50 validation images, and 50 test images. 
For the results presented in Section \ref{sec:Training}, the training images were cropped, rescaled, flipped, and rotated to form a set of 204,800 overlapping $40\times 40$ patches. The validation images were cropped to form 1,000 non-overlapping $40\times 40$ patches. We used $256$ non-overlapping $40\times 40$ patches for test.
For the results presented in this section, we used 382,464 $50\times 50$ patches for training, 6,528 $50\times 50$ patches for validation, and seven standard test images, illustrated in Figure \ref{fig:TestImages} and rescaled to various resolutions, for test.

\begin{figure}[t]
\centering
\subfigure[Barbara]{\includegraphics[width=.135\textwidth]{figs/barbara.png}}
\subfigure[Boat]{\includegraphics[width=.135\textwidth]{figs/boat.png}}
\subfigure[Couple]{\includegraphics[width=.135\textwidth]{figs/couple.png}}
\subfigure[Peppers]{\includegraphics[width=.135\textwidth]{figs/peppers.png}}
\subfigure[Fingerprint]{\includegraphics[width=.135\textwidth]{figs/fingerprint.png}}
\subfigure[Mandrill]{\includegraphics[width=.135\textwidth]{figs/mandrill.png}}
\subfigure[Bridge]{\includegraphics[width=.135\textwidth]{figs/streamandbridge.png}}
\caption{The seven test images.}
\label{fig:TestImages}
\end{figure}

\paragraph{Implementation.}
We implemented LDAMP and LDIT, using the DnCNN denoiser \cite{DnCNN}, in both TensorFlow and MatConvnet \cite{vedaldi15matconvnet}, which is a toolbox for Matlab.
%The MatConvnet implementation of DnCNN was provided by the its authors here \url{https://github.com/cszn/DnCNN}. 
Public implementations of both versions of the algorithm are available at \url{https://github.com/ricedsp/D-AMP_Toolbox}.

\paragraph{Training parameters.}
We trained all the networks using the Adam optimizer \cite{ADAMopt} with a training rate of 0.001, which we dropped to 0.0001 and then 0.00001 when the validation error stopped improving. We used mini-batches of 32 to 256 patches, depending on network size and memory usage. For layer-by-layer and denoiser-by-denoiser training, we used a different randomly generated measurement matrix for each mini-batch.
Training generally took between 3 and 5 hours per denoiser on an Nvidia Pascal Titan X. Results in this section are for denoiser-by-denoiser trained networks which consists of 10 unrolled DAMP/DIT layers that each contain a 20 layer DnCNN denoiser.

\paragraph{Competition.}
We compared the performance of LDAMP to three state-of-the-art image recovery algorithms; TVAL3 \cite{TVAL3}, NLR-CS \cite{NLRCS}, and BM3D-AMP \cite{DAMPITIT}. We also include a comparison with LDIT to demonstrate the benefits of the Onsager correction term.
Our results do not include comparisons with any other NN-based techniques. 
%OneNet \cite{OneNettoSolve} code was not available in time to test it before the deadline. 
%The RIDE-CS \cite{KaushikGenerativeNN} code 
While many NN-based methods are very specialized and only work for fixed matrices \cite{mousaviSDA, reconnet, deepinverse, dr2net, DeepADMMnet}, the recently proposed OneNet \cite{OneNettoSolve} and RIDE-CS \cite{KaushikGenerativeNN} methods can be applied more generally.
Unfortunately, we were unable to train and test the OneNet code in time for this submission. While RIDE-CS code was available, the implementation requires the measurement matrices to have orthonormalized rows. When tested on matrices without orthonormal rows, RIDE-CS performed significantly worse than the other methods. %In addition,  reconstructing a single $128\times128$ image with RIDE-CS took over thirty minutes which made fully testing it impractical.

%Note that although we trained and tested BM3D-VAMP and Learned D-VAMP \cite{DVAMP}, we do not include their results here as their results were nearly

\paragraph{Algorithm parameters.}
All algorithms used their default parameters. However, NLR-CS was initialized using 8 iterations of BM3D-AMP, as described in \cite{DAMPITIT}. BM3D-AMP was run for 10 iterations. LDIT and LDAMP used 10 layers. 
LDIT had its per layer noise standard deviation estimate $\hat{\sigma}$ parameter set to $2\|z^l\|_2/\sqrt{m}$, as was done with D-IT in \cite{DAMPITIT}. 


\paragraph{Testing setup.}
We tested the algorithms with i.i.d.~Gaussian measurements and with measurements from a randomly sampled coded diffraction pattern \cite{candes2015phase}. The coded diffraction pattern forward operator was formed as a composition of three steps; randomly (uniformly) change the phase, take a 2D FFT, and then randomly (uniformly) subsample. 
Except for the results in Figure \ref{fig:VisualComparo}, we tested the algorithms with $128\times 128$ images ($n=128^2$).
%We also tested all recovery algorithms except for NLR-CS with coded diffraction measurements of $512\times 512$ images ($n=512^2$). 
We report recovery accuracy in terms of PSNR. We report run times in seconds. %This section summarizes the recovery results.
Results broken down by image are provided in the supplement.
%\subsection{Results}

%In this section we summarize the results from testing all five algorithms, on all seven test images, at five different sampling rates, with both Gaussian and coded diffraction measurements. These results can be found in table form in the supplement.
%In this section we compare the performance of the various recovery algorithms. Tables \ref{tab:GaussianPSNR} and \ref{tab:GaussianTime} compare the PSNRs and runtimes, respectively, of reconstructions of the 6 test images when the measurements are Gaussian and there is no measurement noise. 
%Table \ref{tab:GaussianPSNR} demonstrates that w

\paragraph{Gaussian measurements.}
With noise-free Gaussian measurements, the  LDAMP network produces the best reconstructions at every sampling rate on every image except Fingerprints, which looks very unlike the natural images the network was trained on.
%Table \ref{tab:GaussianTime} demonstrates that 
With noise-free Gaussian measurements, LDIT and LDAMP produce reconstructions significantly faster than the competing methods. 
Note that, despite having to perform twice as many denoising operations, at a sampling rate of $\frac{m}{n}=0.25$ the LDAMP network is only about $25\%$ slower than LDIT. This indicates that matrix multiplies, not denoising operations, are the dominant source of computation. Average recovery PSNRs and run times are reported in Table \ref{tab:gaussian}. With noisy Gaussian measurements, LDAMP uniformly outperformed the other methods; these results can be found in the supplement.


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{PSNRs and run times (sec) of $128 \times 128$ reconstructions with i.i.d.~Gaussian measurements and no measurement noise at various sampling rates.}
    \begin{tabular}{lrrrrrrrr}
    \toprule
     \multirow{2}{*}{Method}&% \multicolumn{2}{c}{$\frac{m}{n}=.05$} & 
     \multicolumn{2}{c}{{$\frac{m}{n}=0.10$}} & \multicolumn{2}{c}{$\frac{m}{n}=0.15$} & \multicolumn{2}{c}{$\frac{m}{n}=0.20$} & \multicolumn{2}{c}{$\frac{m}{n}=0.25$} \\
    \cmidrule{2-9} %\cmidrule{4-5}% \cmidrule{1-2} \cmidrule{1-2} \cmidrule{1-2}
     %& PSNR & Time 
     & PSNR & Time & PSNR & Time & PSNR & Time & PSNR & Time \\
    \midrule
    TVAL3 & %19.8 & 1.4  &
    21.5 & 2.2  & 22.8 & 2.9  & 24.0 & 3.6  & 25.0 & 4.3 \\
    BM3D-AMP & %17.9 & 3.8  &
    23.1 & 4.8  & 25.1 & 4.4  & 26.6 & 4.2  & 27.9 & 4.1 \\
    LDIT & %18.4 & 0.2  &
    20.1 & \textbf{0.3}  & 20.7 & \textbf{0.4} & 21.1 & \textbf{0.4} & 21.7 & \textbf{0.5} \\
    LDAMP & %21.1 & 0.3  &
    \textbf{23.7} & 0.4  & \textbf{25.7} & 0.5  & \textbf{27.2} & 0.5  & \textbf{28.5} & 0.6 \\
    NLR-CS & %19.9 & 67.8  &
    23.2 & 85.9  & 25.2 & 104.0  & 26.8 & 124.4  & 28.2 & 146.3 \\
    \bottomrule
    \end{tabular}%
  \label{tab:gaussian}%
\end{table}%


% \paragraph{Noisy Gaussian measurements.}
%  With noisy Gaussian measurements LDAMP uniformly outperformed the other methods.\footnote{We did not test NLR-CS with noisy measurements because \cite{DAMPITIT} demonstrated than in the presence of noise BM3D-AMP significantly outperforms NLR-CS.} Tables with recovery results, includign results in the presence of noise, can be found in the supplement.

% \begin{table}[t]
%   \centering
%   \caption{PSNR of reconstruction of $128 \times 128$ Boat test image with additive white Gaussian measurement noise (AWGN) with various standard deviations  (s.d.).}
%     \begin{tabular}{lrrrrrrrrrr}
%     \toprule
%      \multirow{2}{*}{Method}& \multicolumn{2}{c}{\textbf{5\%}} & \multicolumn{2}{c}{\textbf{10\%}} & \multicolumn{2}{c}{\textbf{15\%}} & \multicolumn{2}{c}{\textbf{20\%}} & \multicolumn{2}{c}{\textbf{25\%}} \\
%     \cmidrule{2-11} %\cmidrule{4-5}% \cmidrule{1-2} \cmidrule{1-2} \cmidrule{1-2}
%      & PSNR & Time & PSNR & Time & PSNR & Time & PSNR & Time & PSNR & Time \\
%     \midrule
%     TVAL3 & 19.8 & 1.4  & 21.5 & 2.2  & 22.8 & 2.9  & 24.0 & 3.6  & 25.0 & 4.3 \\
%     D-AMP & 17.9 & 3.8  & 23.1 & 4.8  & 25.1 & 4.4  & 26.6 & 4.2  & 27.9 & 4.1 \\
%     LDIT & 18.4 & 0.2  & 20.1 & 0.3  & 20.7 & 0.4  & 21.1 & 0.4  & 21.7 & 0.5 \\
%     LDAMP & 21.1 & 0.3  & 23.7 & 0.4  & 25.7 & 0.5  & 27.2 & 0.5  & 28.5 & 0.6 \\
%     NLR-CS & 19.9 & 67.8  & 23.2 & 85.9  & 25.2 & 104.0  & 26.8 & 124.4  & 28.2 & 146.3 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:noisy}%
% \end{table}%


%Tables \ref{tab:CodedDiffractionPSNR} and \ref{tab:CodedDiffractionTime} compare the PSNRs and runtimes, respectively, of reconstructions of the 6 test images when the measurements are subsampled coded diffraction patterns and there is no measurement noise. 

\paragraph{Coded diffraction measurements.}
% Table \ref{tab:CodedDiffractionPSNR} demonstrates that 
With noise-free coded diffraction measurements, the LDAMP network again produces the best reconstructions on every image except Fingerprints. 
% Table \ref{tab:CodedDiffractionTime} demonstrates that 
With coded diffraction measurements, LDIT and LDAMP produce reconstructions significantly faster than competing methods. 
Note that because the coded diffraction measurement forward and backward operator can be applied in $O(n\log n)$ operations, denoising becomes the dominant source of computations: LDAMP, which has twice as many denoising operations as LDIT, takes roughly $2\times$ longer to complete. 
Average recovery PSNRs and run times are reported in Table \ref{tab:diffraction}.
We end this section with a visual comparison of $512\times 512$ reconstructions from TVAL3, BM3D-AMP, and LDAMP, presented in Figure \ref{fig:VisualComparo}. At high resolutions, the LDAMP reconstructions are incrementally better than those of BM3D-AMP yet computed over $60\times$ faster. 

\begin{table}[t]
  \centering
  \caption{PSNRs and run times (sec) of $128 \times 128$ reconstructions with coded diffraction measurements and no measurement noise at various sampling rates.}
    \begin{tabular}{lrrrrrrrr}
    \toprule
     \multirow{2}{*}{Method}&% \multicolumn{2}{c}{$\frac{m}{n}=0.05$} & 
     \multicolumn{2}{c}{{$\frac{m}{n}=0.10$}} & \multicolumn{2}{c}{$\frac{m}{n}=0.15$} & \multicolumn{2}{c}{$\frac{m}{n}=0.20$} & \multicolumn{2}{c}{$\frac{m}{n}=0.25$} \\
    \cmidrule{2-9} %\cmidrule{4-5}% \cmidrule{1-2} \cmidrule{1-2} \cmidrule{1-2}
     %& PSNR & Time 
     & PSNR & Time & PSNR & Time & PSNR & Time & PSNR & Time \\
    \midrule
    TVAL3 & %21.5 & 0.62  &
    24.0 & 0.52  & 26.0 & 0.46  & 27.9 & 0.43  & 29.7 & 0.41 \\
    BM3D-AMP & %16.9 & 3.80  &
    23.8 & 4.55  & 25.7 & 4.29  & 27.5 & 3.67  & 29.1 & 3.40 \\
    LDIT & %20.0 & 0.13  &
    22.9 & \textbf{0.14} & 25.6 & \textbf{0.14}  & 27.4 & \textbf{0.14}  & 28.9 & \textbf{0.14} \\
    LDAMP & %21.9 & 0.26  &
    \textbf{25.3} & 0.26  & \textbf{27.4} & 0.26  & \textbf{28.9} & 0.27  & \textbf{30.5} & 0.26 \\
    NLR-CS & %15.7 & 87.26  &
    21.6 & 87.82  & 22.8 & 87.43  & 25.1 & 87.18  & 26.4 & 86.87 \\
    \bottomrule
    \end{tabular}%
  \label{tab:diffraction}%
\end{table}%

\begin{figure}[ht]
\centering
\subfigure[Original Image]{\includegraphics[width=.24\textwidth]{figs/boat_zoomed.png}} %26.4 dB
\subfigure[TVAL3 (26.4 dB, 6.85 sec)]{\includegraphics[width=.24\textwidth]{figs/Boat512_TVAL3_5percent_zoomed.png}} %26.4 dB
\subfigure[BM3D-AMP (27.2 dB, 75.04 sec)]{\includegraphics[width=.24\textwidth]{figs/Boat512_BM3DAMP_5percent_zoomed.png}} %27.2 dB, 
\subfigure[LDAMP (28.1 dB, 1.22 sec)]{\includegraphics[width=.24\textwidth]{figs/Boat512_LearnedDAMP_5percent_zoomed.png}} %28.1 dB
\caption{Reconstructions of $512 \times 512$ Boat test image sampled at a rate of $\frac{m}{n}=0.05$ using coded diffraction pattern measurements and no measurement noise. LDAMP's reconstructions are noticeably cleaner and far faster than the competing methods. % \richb{can you fix the a  b c d spilling over 2 lines?}
}
\label{fig:VisualComparo}
\end{figure}



%Test networks trained at a specific sampling rate vs networks trained at lots of sampling rates.

==> Learned D-AMP NIPS 2017_arxiv/Intro.tex <==
\section{Introduction}

Over the last few decades computational imaging systems have proliferated in a host of different imaging domains, from synthetic aperture radar to functional MRI and CT scanners. The majority of these systems capture linear measurements $y\in\mathbb{R}^m$ of the signal of interest $x\in \mathbb{R}^n$ via $y=\mathbf{A}x+\epsilon$, where $\mathbf{A}\in\mathbb{R}^{m\times n}$ is a measurement matrix and $\epsilon\in\mathbb{R}^m$ is noise.
%\footnote{Analogous equations can be written when dealing with complex-valued signals and measurements.}

Given the measurements $y$ and the measurement matrix $A$, a computational imaging system seeks to recover $x$.
When $m<n$ this problem is underdetermined, and prior knowledge about $x$ must be used to recovery the signal. This problem is broadly referred to as {\em compressive sampling} (CS) \cite{CandesRobust, baraniuk2007compressive}.

% Recovering compressively sampled images presents two central challenges.
% First, the dimensions of typical images are on the order of hundreds of thousands to millions.
% Thus any algorithm that we hope to run in anywhere close to real time must be extremely efficient.
% Second, images have complicated structures which necessitate sophisticated priors. Simple models like sparsity produce poor reconstructions \cite{DAMPITIT}.

% Recently neural networks (NN) have made strides towards solving both of these problems \cite{mousaviSDA, reconnet, deepinverse, dr2net, DeepADMMnet,KaushikGenerativeNN, OneNettoSolve}.
% First, through the effective use of massively parallel GPU architectures they are able to run orders of magnitude faster than existing compressive image recovery methods.
% Second, by using vast amounts of training data they are able to implicitly learn accurate models for natural images.
 
% Unfortunately, NNs come with drawbacks. They are difficult to train, often-times specific to a single measurement matrix, and largely unprincipled blackboxes. This work rectifies these problems by creating networks that mimic the behavior of Denoising-based AMP (D-AMP) \cite{DAMPITIT} and Denoising-based VAMP (D-VAMP) \cite{DVAMP}; algorithms with exceptional performance and well known characteristics.

% The inspiration for this work comes from the LISTA \cite{LISTA, kamilov2016learning} and LAMP/LVAMP \cite{LAMP} neural networks. In these works, the authors unroll the iterative ISTA \cite{ISTA} and AMP/VAMP \cite{DoMaMo09, VAMP} algorithms, respectively, and then treat parameters of the algorithm as weights to be learned. In this way, an algorithm consisting of $L$ iterations become a neural network with $L$ layers. We do the same to D-AMP and D-VAMP to form Learned D-AMP (LDAMP) and Learned D-VAMP (LDVAMP). However, whereas the LISTA and LAMP/LVAMP networks efficiently recover compressively sampled sparse signals, LDAMP and LDVAMP recover compressively sampled images.

% Because they are based off of the well understood D-AMP and D-VAMP algorithms, LDAMP/LDVAMP are easy to train, can be applied to a variety of different measurement matrices, and come with a state-evolution heuristic that accurately predicts their performance. Most importantly, LDAMP/LDVAMP outperform the state-of-the-art BM3D-AMP and NLR-CS algorithms in terms of both accuracy and runtime. 
% At high resolutions, when used with matrices which have fast matrix multiply implementations, LDAMP runs over $50\times$ faster than BM3D-AMP and hundreds of times faster than NLR-CS.

There are myriad ways to use priors to recover an image $x$ from compressive measurements. 
In the following, we briefly describe some of these methods. Note that the ways in which these algorithms use priors span a spectrum; from simple hand-designed models to completely data-driven methods (see Figure \ref{fig:related_works}).

\begin{figure}[H]
\begin{center}
\includegraphics[width=11cm]{figs/SpectrumofAlgs_2_noLDVAMP.png}
\caption{ The spectrum of compressive signal recovery algorithms.  %\richb{if you have time put arrows on the end of the spectrum?  or is it a balance beam?}\cm{I used three lines because there are meant to be three supersets. Ideally the simple models would be on top of the complicated models but there wasn't room.}
}
\label{fig:related_works}
\end{center}
\end{figure}

\subsection{Hand-designed recovery methods}
%One approach for solving \eqref{eq:l0} is to replace $\ell_0$-norm with its convex relaxed version which is $\ell_1$-norm. 
The vast majority of CS recovery algorithms can be considered ``hand-designed'' in the sense that they use some sort of expert knowledge, i.e., prior, about the structure of $x$.
The most common signal prior is that $x$ is sparse in some basis. 
Algorithms using sparsity priors include CoSaMP \cite{TroppNeedellCoSaMP}, ISTA \cite{ISTA}, approximate message passing (AMP) \cite{DoMaMo09}, and VAMP \cite{VAMP}, among many others. 
Researchers have also developed priors and algorithms that more accurately describe the structure of natural images, such as minimal total variation, e.g., TVAL3 \cite{TVAL3}, markov-tree models on the wavelet coefficients, e.g., Model-CoSaMP \cite{RichModelBasedCS}, and nonlocal self-similarity, e.g., NLR-CS \cite{NLRCS}. Off-the-shelf denoising and compression algorithms have also been used to impose priors on the reconstruction, e.g., Denoising-based AMP (D-AMP) \cite{DAMPITIT}, D-VAMP \cite{DVAMP}, and C-GD \cite{ArianCompressionbased}. When applied to natural images, algorithms using advanced priors outperform simple priors, like wavelet sparsity, by a large margin \cite{DAMPITIT}.


The appeal of hand-designed methods is that they are based on interpretable priors and often have well understood behavior. Moreover, when they are set up as convex optimization problems they often have theoretical convergence guarantees. 
Unfortunately, among the algorithms that use accurate priors on the signal, even the fastest is too slow for many real-time applications \cite{DAMPITIT}.
More importantly, these algorithms do not take advantage of potentially available training data. As we will see, this leaves much room for improvement.

% These hand-designed approaches have a few major benefits. 
% First, because they are typically solutions to a convex optimization methods, they often have theoretical convergence guarantees. 
% Second, they do not rely on training data and are universal in that sense. Unfortunately, they are often slow to converge and hence are not suitable for real time applications of CS. 

%Furthermore, they are rarely designed specifically for a particular application and thus their performance is not optimized in that sense.

\subsection{Data-driven recovery methods}

At the other end of the spectrum are data-driven (often deep learning-based) methods that use no hand-designed models whatsoever. %That is, the algorithms themselves are completely agnostic to any prior we might have about the signal.
Instead, researchers provide neural networks (NNs) vast amounts of training data, and the networks learn how to best use the structure within the data \cite{mousaviSDA, reconnet, deepinverse, dr2net}.

The first paper to apply this approach was \cite{mousaviSDA}, where the authors used stacked denoising autoencoders (SDA) \cite{SDA} to recover signals from their undersampled measurements. Other papers in this line of work have used either pure convolutional layers (DeepInverse \cite{deepinverse}) or a combination of convolutional and fully connected layers (DR$^2$-Net \cite{dr2net} and ReconNet \cite{reconnet}) to build deep learning frameworks capable of solving the CS recovery problem. As demonstrated in \cite{mousaviSDA}, these methods can compete with state-of-the-art methods in terms of accuracy while running thousands of times faster. Unfortunately, these methods are held back by the fact that there exists almost no theory governing their performance and that, so far, they must be trained for specific measurement matrices and noise levels.

\subsection{Mixing hand-designed and data-driven methods for recovery}
\label{ssec:mixedmethods}

The third class of recovery algorithms blends data-driven models with hand-designed algorithms. 
These methods first use expert knowledge to set up a recovery algorithm and then use training data to learn priors within this algorithm.
Such methods benefit from the ability to learn more realistic signal priors from the training data, while still maintaining the interpretability and guarantees that made hand-designed methods so appealing. 
Algorithms of this class can be divided into two subcategories. The first subcategory uses a black box neural network that performs some function within the algorithm, such as the proximal mapping.
The second subcategory explicitly unrolls and iterative algorithm and turns it into a deep NN.
Following this unrolling, the network can be tuned with training data.
Our LDAMP algorithm uses ideas from both these camps.


\paragraph{Black box neural nets.}
The simplest way to use a NN in a principled way to solve the CS problem is to treat it as a black box that performs some function; such as computing a posterior probability. Examples of this approach include RBM-AMP and its generalizations \cite{RBM_AMP, GRBM_AMP, GRBM_AMP_Journal}, which use Restricted Boltzmann Machines to learn non-i.i.d.~priors; RIDE-CS \cite{KaushikGenerativeNN}, which uses the RIDE \cite{RIDE} generative model to compute the probability of a given estimate of the image; and OneNet \cite{OneNettoSolve}, which uses a NN as a proximal mapping/denoiser.

% The first examples of this approach showed up in a series of works, \cite{RBM_AMP, GRBM_AMP, GRBM_AMP_Journal}, which integrated Restricted Boltzmann Machines (RBM) into the AMP algorithm. The resulting algorithms, RBM-AMP and its generalizations, use RBMs to learn and apply non-i.i.d.~priors to solve the CS problem.
% When trained on the MNIST dataset, the algorithms were able to successfully model and use the correlations within images of handwritten digits.

% The second example of this approach, which we denote as RIDE-CS, was developed in \cite{KaushikGenerativeNN}. In this work the authors used the RIDE \cite{RIDE} generative model to compute the probability of a given estimate of the image. This enabled them to use gradient ascent on the signal's posterior distribution to reconstruct images from compressive measurements.

% The third method, which we denote OneNet \cite{OneNettoSolve}, uses ADMM %\cite{boyd2011distributed}
% to solve several imaging inverse problems including inpainting, denoising, and CS. This method uses a NN as a proximal mapping, and can be interpreted as a NN-based version of Plug and Play ADMM \cite{PlugandPlayADMM}. Using a NN in this way allows the authors to derive useful convergence guarantees.

\paragraph{Unrolled algorithms.}
The second way to use a NN in a principled way to solve the CS problem is to simply take a well-understood iterative recovery algorithm and unroll/unfold it. This method is best illustrated by the the LISTA \cite{LISTA, kamilov2016learning} and LAMP \cite{LAMP} NNs. In these works, the authors simply unroll the iterative ISTA \cite{ISTA} and AMP \cite{DoMaMo09} algorithms, respectively, and then treat parameters of the algorithm as weights to be learned. %One can parameterize the matrices $\mathbf{A}$ and $\mathbf{A}^H$ \cite{LISTA}, the nonlinearities $\eta_\theta(\cdot)$ \cite{kamilov2016learning}, or both \cite{LAMP}. 
Following the unrolling, training data can be fed through the network, and stochastic gradient descent can be used to update and optimize its parameters.
% \begin{multicols}{2}
% \begin{tcolorbox}
% AMP Algorithm
% \begin{align}%\label{eqn:amp}
% z^t &= y -\mathbf{A}\hat{x}^t + \frac{\|\hat{x}^{t}\|_0}{m}z^{t-1}, \nonumber \\
% \hat{x}^{t+1} &= \eta_{\theta^{t}}(\hat{x}^t + \mathbf{A}^H z^t; \frac{ \|z^t\|_2}{\sqrt{m}}). \nonumber
% \end{align}
% \end{tcolorbox}
% \begin{tcolorbox}
% Learned AMP (LAMP) Neural Network
% \begin{align}%\label{eqn:lamp}
% z^0 &= y -\mathbf{A}\hat{x}^0 \nonumber \\
% \hat{x}^{1} &= \eta_{\theta^{1}}(\hat{x}^0 + \mathbf{A}^H z^0; \frac{ \|z^0\|_2}{\sqrt{m}}), \nonumber \\
% z^1 &= y -\mathbf{A}\hat{x}^1 + \frac{\|\hat{x}^{1}\|_0}{m}z^0, \nonumber \\
% \hat{x}^{2} &= \eta_{\theta^{2}}(\hat{x}^1 + \mathbf{A}^H z^1; \frac{ \|z^1\|_2}{\sqrt{m}}), \nonumber \\
% &\vdots \nonumber \\
% \hat{x}^{L} &= \eta_{\theta^{L}}(\hat{x}^{L-1} + \mathbf{A}^H z^{L-1}; \frac{ \|z^{L-1}\|_2}{\sqrt{m}}). \nonumber
% \end{align}
% \end{tcolorbox}
% \end{multicols}
% To be concrete, consider AMP and LAMP. % AMP solves the CS problem through the following iterations.
% In the AMP algorithm $ \eta(\cdot)_{\theta^{t}}$ is some simple nonlinearity, such as soft-thresholding, parameterized by ${\theta^{t}}$. The terms $x^t$ and $z^t$ are the estimates of the signal $x$ and the residual $z$ at iteration $t$.
% In the LAMP network, the authors simply unroll the iterations of AMP.
% The equations to the right now define a neural network. Training data can be fed through it and stochastic gradient descent can be used to update and optimize its parameters ${\theta^{0}}, {\theta^{1}}, ...$ .
% %AMP usually converges in tens to hundreds of iterations, LAMP converges in far fewer \cite{LAMP}.
Unrolling was recently applied to the ADMM algorithm to solve the CS-MRI problem \cite{DeepADMMnet}. The resulting network, ADMM-Net, uses training data to learn filters, penalties, simple nonlinearities, and multipliers. 
Moving beyond CS, the unrolling principle has been applied successfully in speech enhancement \cite{deepunfolding}, non-negative matrix factorization applied to music transcription \cite{yakar2013bilevel}, and beyond.
In these applications, unrolling and training significantly improve both the quality and speed of signal reconstruction.
% Our goal in this work is to design a method that benefits from $\ell_1$-minimization problem and at the same time uses the benefits of pure data-driven approaches. We mix ideas from D-AMP and convolutional neural networks to design a new CS recovery algorithm. This combination will let us to have a theoretical framework for the performance of our algorithm and at the same time use the major benefit of deep learning frameworks that is ultra-fast recovery. We show that our designed algorithm outperforms state-of-the-art methods in quality and speed of signal reconstruction. 


==> Learned D-AMP NIPS 2017_arxiv/LDAMPsection.tex <==
\section{Learned D-AMP}
% In this section we first briefly review the denoising-based iterative thresholding (D-IT) and denoising-based AMP (D-AMP) \cite{DAMPITIT} algorithms. We then describe the denoising convolutional neural network (DnCNN) image denoiser \cite{DnCNN}. Finally, we describe how D-IT and D-AMP can be unrolled and combined with the DnCNN denoiser to form Learned D-IT (LDIT) and Learned D-AMP (LDAMP).

\subsection{D-IT and D-AMP}\label{ssec:DAMP}

% \begin{multicols}{2}
%\begin{vwcol}[widths={0.2,0.8}, sep=0cm, justify=flush,rule=0pt,indent=1em] 

%\end{vwcol}
% \end{multicols}

\begin{figure}[t]
\centering
\subfigure[D-IT Iterations]{\includegraphics[width=.35\textwidth]{figs/AlgorithmBehaviorDiagrams_DIT_2.png}}
\hspace*{15mm}
\subfigure[D-AMP Iterations]{\includegraphics[width=.35\textwidth]{figs/AlgorithmBehaviorDiagrams_DAMP_2.png}}
  \caption{Reconstruction behavior of D-IT (left) and D-AMP (right) with an idealized denoiser. Because D-IT allows bias to build up over iterations of the algorithm, its denoiser becomes ineffective at projecting onto the set ${C}$ of all natural images. The Onsager correction term enables D-AMP to avoid this issue. Figure adapted from \cite{DAMPITIT}.}
   \label{fig:DAMPBehavior}
\end{figure}


% \subsubsection{Image Denoisers}
% \subsubsection{Denoising-based Iterative Thresholding}

{\em Learned D-AMP} (LDAMP), is a mixed hand-designed/data-driven compressive signal recovery framework that is builds on the D-AMP algorithm \cite{DAMPITIT}.
We describe D-AMP now, as well as the simpler denoising-based iterative thresholding (D-IT) algorithm.  
For concreteness, but without loss of generality, we focus on image recovery.


%To understand the D-IT and D-AMP algorithms, it helps to formulate the compressive imaging problem as follows. Let $C$ denote the set of all natural images. 

A compressive image recovery algorithm solves the ill-posed inverse problem of finding the image $x$ given the low-dimensional measurements $y= \mathbf{A} x$ by exploiting prior information on $x$, such as fact that $x\in C$, where $C$ is the set of all natural images.
A natural optimization formulation reads
\begin{align}\label{eqn:CompressiveImagingProblem}
    \text{argmin}_x \|y -\mathbf{A} x \|_2^2 \text{~~subject to~~} x\in C. 
\end{align}
When no measurement noise $\epsilon$ is present, a compressive image recovery algorithm should return the (hopefully unique) image $x_o$ at the intersection of the set $C$ and the affine subspace $\{x|y= \mathbf{A}x\}$ (see Figure \ref{fig:DAMPBehavior}).

The premise of D-IT and D-AMP is that high-performance image denoisers $D_\sigma$, such as BM3D \cite{DabovBM3D}, are high-quality approximate projections onto the set $C$ of natural images.\footnote{The notation $D_\sigma$ indicates that the denoiser can be parameterized by the standard deviation of the noise $\sigma$.}$^{,}$\footnote{Denoisers can also be thought of as a proximal mapping with respect to the negative log likelihood of natural images \cite{venkatakrishnan2013plug} or as taking a gradient step with respect to the data generating function of natural images \cite{BengioDenosier, sonderby2016amortised}.} 
That is, suppose $x_o+\sigma z$ is a noisy observation of a natural image, with $x_o\in C$ and $z\sim N(0,I)$. An ideal denoiser $D_\sigma$ would simply find the point in the set $C$ that is closest to the observation $x_o+\sigma z$
%
\begin{align}\label{eqn:DenoisingProblem}
D_\sigma(x)=\text{argmin}_x \|x_o+\sigma z - x \|_2^2 \text{~~subject to~~} x\in C. 
\end{align}

Combining \eqref{eqn:CompressiveImagingProblem} and \eqref{eqn:DenoisingProblem} leads naturally to the D-IT algorithm, presented in \eqref{eqn:DIT} and illustrated in Figure \ref{fig:DAMPBehavior}(a).
Starting from $x^0=0$, D-IT takes a gradient step towards the $\{x|y= \mathbf{A}x\}$ affine subspace and then applies the denoiser $D_\sigma$ to move to $x^1$ in the set $C$ of natural images . 
Gradient stepping and denoising is repeated for $t=1,2,\dots$ until convergence.

\begin{tcolorbox}
D-IT Algorithm
\vspace{-6 mm}
\begin{eqnarray}\label{eqn:DIT}
z^t&=& y-\mathbf{A}x^t, \nonumber \\%+z^{t-1} \frac{{\rm div} D_{\hat{\sigma}^{t-1}}(x^{t-1}+\mathbf{A}^Hz^{t-1})}{m}. \nonumber \\
x^{t+1} &=& D_{\hat{\sigma}^t} (x^t+\mathbf{A}^Hz^t). 
\end{eqnarray}
\end{tcolorbox}

Let $\nu^t=x^t+\mathbf{A}^Hz^t-x_o$ denote the difference between $x^t+\mathbf{A}^Hz^t$ and the true signal $x_o$ at each iteration. $\nu^t$ is known as the {\em effective noise}.
At each iteration, D-IT denoises  $x^t+\mathbf{A}^Hz^t=x_o+\nu^t$, i.e., the true signal plus the effective noise. 
Most denoisers are designed to work with $\nu^t$ as additive white Gaussian noise (AWGN). 
Unfortunately, as D-IT iterates, the denoiser biases the intermediate solutions, and $\nu^t$ soon deviates from AWGN.
Consequently, the denoising iterations become less effective \cite{DoMaMo09, DAMPITIT, LAMP}, and convergence slows. 
%This behavior is best demonstrated with iterative soft-thresholding (IST) \cite{FiNoWr07}, the simplest version of D-IT. IST has a well documented behaviour of producing heavy-tailed, nongaussian effective noise \cite{DoMaMo09, DAMPITIT, LAMP}.

%\subsection{Denoising-based AMP}\label{ssec:DAMP}


D-AMP differs from D-IT in that it corrects for the bias in the effective noise at each iteration $t=0,1,\dots$ using an {\em Onsager correction} term $b^t$.
%
\begin{tcolorbox}
D-AMP Algorithm
\vspace{-6 mm}
\begin{eqnarray}\label{eqn:DAMP}
b^t&=& \frac{z^{t-1} {\rm div} D_{\hat{\sigma}^{t-1}}(x^{t-1}+\mathbf{A}^Hz^{t-1})}{m}, \nonumber \\
z^t&=& y-\mathbf{A}x^t+b^t, \nonumber \\
\hat{\sigma}^t&=& \frac{\|z^t\|_2}{\sqrt{m}}, \nonumber \\
x^{t+1} &=& D_{\hat{\sigma}^t} (x^t+\mathbf{A}^Hz^t). 
\end{eqnarray}
\end{tcolorbox}
%
%D-AMP, presented in \eqref{eqn:DAMP}, is no more than the D-IT algorithm plus an Onsager correction term; $b^t$. %$z^{t-1} \frac{{\rm div} D_{\hat{\sigma}^{t-1}}(x^{t-1}+\mathbf{A}^Hz^{t-1})}{m}$.
%\footnote{${\rm div} D(\cdot)$ denotes the divergence of the denoiser: the sum of $D(\cdot)$'s partial derivatives with respect to $x$.}
The Onsager correction term removes the bias from the intermediate solutions so that the effective noise $\nu^t$ follows the AWGN model expected by typical image denoisers. 
%A derivation of where the Onsager correction term came from is beyond the scope of this work. 
For more information on the Onsager correction, its origins, and its connection to the Thouless-Anderson-Palmer equations \cite{thouless1977solution}, see \cite{DoMaMo09} and \cite{MezardMontanari}. 
Note that $\frac{\|z^t\|_2}{\sqrt{m}}$ serves as a useful and accurate estimate of the standard deviation of $\nu^t$ \cite{MalekiThesis}.
Typically, D-AMP algorithms use a Monte-Carlo approximation for the divergence ${\rm div} D(\cdot)$, which was first introduced in \cite{RamaniMCSure, DAMPITIT}.
%\footnote{When the divergence can be computed analytically D-AMP is just AMP.}

% Given a denoiser $D_{\hat{\sigma}}(x)$, using an i.i.d. random vector $b \sim N(0,I)$, we can estimate the divergence with
% \begin{eqnarray}
% \label{eqn:div_est}
% {\rm div} D_{\hat{\sigma}}&=&\lim\limits_{\epsilon\rightarrow 0}E_{b} \left\{b^{*}\left(\frac{D_{\hat{\sigma}}(x+\epsilon b)-D_{\hat{\sigma}}(x)}{\epsilon}\right)\right\}\\ &\approx& \mathbb{E} \left( \frac{1}{\epsilon}b^{*}(D_{\hat{\sigma}}(x+\epsilon b)-D_{\hat{\sigma}}(x))  \right)\text{, for very small $\epsilon$.\nonumber} 
% \end{eqnarray}
% To compute this expected value we can use Monte Carlo sampling:
% \[
% {\rm div} \hat{D}_{\hat{\sigma}^l} = \frac{1}{M} \sum_{i=1}^M \widehat{\rm div}^i, 
% \]
% where $\widehat{\rm div}^i$ is the estimate of the divergence from the $i^{th}$ Monte Carlo sample. 
% In this work set $\epsilon=\frac{\|x\|_\infty}{1000}$ and $M=1$. For more information on this approximation see \cite{DAMPITIT}.

\subsection{Denoising convolutional neural network}

% \begin{figure}[t]
%  \begin{center}
%  	%\begin{center}
%  	% Requires \usepackage{graphicx} 
%  	%\vspace{-1cm}
%  	\includegraphics[width=.95\textwidth]{./figs/DnCNN.png} 
%  	%\vspace{-1.5cm}
%  	\caption{Network architecture of the DnCNN denoiser \cite{DnCNN}. Notice it first estimates the residual, rather than the denoised image itself.}
%  	\label{fig:DnCNN} 
%  \end{center}
% \end{figure}

NNs have a long history in signal denoising; see, for instance \cite{CanNNsbeatBM3D}. However, only recently have they begun to significantly outperform established methods like BM3D \cite{DabovBM3D}. In this section we review the recently developed Denoising Convolutional Neural Network (DnCNN) image denoiser \cite{DnCNN}, which is both more accurate and far faster than competing techniques.

%The DnCNN neural network is illustrated in Figure \ref{fig:DnCNN}. 
The DnCNN neural network consists of 16 to 20 convolutional layers, organized as follows.
The first convolutional layer uses 64 different $3\times 3\times c$ filters (where $c$ denotes the number of color channels) and is followed by a rectified linear unit (ReLU) \cite{Relu}. 
The next 14 to 18 convolutional layers each use $64$ different $3\times3\times64$ filters which are each followed by batch-normalization \cite{batchnorm} and a ReLU.
The final convolutional layer uses $c$ separate $3\times 3\times 64$ filters to reconstruct the signal. 
The parameters are learned via residual learning \cite{residuallearning}.% That is, in the context of the denoising problem \eqref{eqn:DenoisingProblem}, the network is given $x_o+\sigma z$ as an input and produces $\sigma\hat{z}$, not $\hat{x_o}$, as an output. 
%Throughout the rest of this paper, we will use the 20 layer version of the DnCNN network.

% Rather than learning a mapping from a noisy image to a denoised image directly, the DnCNN authors found it beneficial to learn the residual vector.
% That is, in the context of the denoising problem \eqref{eqn:DenoisingProblem}, the network is given $x_o+\sigma z$ as an input and produces $\hat{z}$, not $\hat{x_o}$, as an output. 
% %The benefit of this approach is that the network is trained to remove the highly structured natural image, rather than the unstructured noise. 
% This method, known as residual learning \cite{residuallearning}, sets up the network to remove the highly structured natural image, rather than the unstructured noise; an easier problem. As a result, residual learning improves both the training times and accuracy of the network.%, thereby making DnCNN a prime candidate for use in our LDAMP network.
 
\subsection{Unrolling D-IT and D-AMP into networks}

%\richb{some places you have LDAMP, some places L-DAMP.  choose one.}



% The central contribution of this work is to take the unrolling ideas behind LISTA \cite{LISTA, kamilov2016learning} and LAMP \cite{LAMP} and apply them to D-IT and D-AMP. To reiterate, in \cite{LISTA, kamilov2016learning} and \cite{LAMP} the authors unroll the iterative ISTA \cite{ISTA} and AMP \cite{DoMaMo09} algorithms, respectively, and then treat parameters of the algorithm as weights to be learned. In this way, an algorithm consisting of $L$ iterations become a neural network with $L$ layers. Here we do the same to D-IT and D-AMP to form LDIT and LDAMP. However, whereas the LISTA and LAMP networks efficiently recover compressively sampled sparse signals, LDIT and LDAMP recover compressively sampled images.

 \begin{figure}[t]
 	\begin{center}
 		%\begin{center}
 		% Requires \usepackage{graphicx} 
 		%\vspace{-1cm}
 		\includegraphics[width=1.0\textwidth]{./figs/LDAMP_network.png} 
 		\vspace{-3mm}
 		\caption{Two layers of the LDAMP neural network. When used with the DnCNN denoiser, each denoiser block is a 16 to 20 convolutional-layer neural network. The forward and backward operators are represented as the matrices $\mathbf{A}$ and $\mathbf{A}^H$; however function handles work as well. %This schematic is derived from the one present in \cite{LAMP}.
 		}\label{fig:LDAMPNetwork} 
 	\end{center}
 \end{figure}

The central contribution of this work is to apply the unrolling ideas described in Section \ref{ssec:mixedmethods} to D-IT and D-AMP to form the LDIT and LDAMP neural networks.
The LDAMP network, presented in \eqref{eqn:LDAMP} and illustrated in Figure \ref{fig:LDAMPNetwork}, consists of 10 AMP layers where each AMP layer contains two denoisers with tied weights. One denoiser is used to update $x^l$, and the other is used to estimate the divergence using the Monte-Carlo approximation from \cite{RamaniMCSure, DAMPITIT}. The LDIT network is nearly identical but does not compute an Onsager correction term and hence, only applies one denoiser per layer. One of the few challenges to unrolling D-IT and D-AMP is that, to enable training, we must use a denoiser that easily propagates gradients; a black box denoiser like BM3D will not work. This restricts us to denoisers such as DnCNN, which, fortunately, offers improved performance.

\begin{tcolorbox}
LDAMP Neural Network
\vspace{-3 mm}
\begin{eqnarray}\label{eqn:LDAMP}
b^l&=& \frac{z^{l-1} {\rm div} D^l_{w^{l-1}(\hat{\sigma}^{l-1})}(x^{l-1}+\mathbf{A}^Hz^{l-1})}{m}, \nonumber \\
z^l&=& y-\mathbf{A}x^l+b^l, \nonumber \\
\hat{\sigma}^l&=& \frac{\|z^l\|_2}{\sqrt{m}}, \nonumber \\
x^{l+1} &=& D^{l}_{w^l(\hat{\sigma}^l)} (x^l+\mathbf{A}^Hz^l).
\end{eqnarray}
\end{tcolorbox}

Within \eqref{eqn:LDAMP}, we use the slightly cumbersome notation $D^{l}_{w^l(\hat{\sigma}^l)}$ to indicate that layer $l$ of the network uses denoiser $D^l$, that this denoiser depends on its weights/biases $w^l$, and that these weights may be a function of the estimated standard deviation of the noise $\hat{\sigma}^l$. %In practice one need not use a different denoiser at different layers, and in fact we found it easiest to train and use a single denoiser, whose weights were set by $\hat{\sigma}^l$, for all the layers.
During training, the only free parameters we learn are the denoiser weights $w^{1},...w^{L}$. 
This is distinct from the LISTA and LAMP networks, where the authors decouple and learn the $\mathbf{A}$ and $\mathbf{A}^H$ matrices used in the network \cite{LISTA,LAMP}.% from the true measurement matrix, which may not be exactly known, and learn them on a layer-by-layer basis \cite{LISTA, LAMP}. Because our focus is on high-dimensional imaging problems, where the measurement matrices can have many millions of elements, we did not pursue this direction and kept our forward and backward operators, $\mathbf{A}$ and $\mathbf{A}^H$ known and fixed. In \cite{kamilov2016learning} the authors also fixed $\mathbf{A}$ and $\mathbf{A}^H$ and just optimized the nonliearities used in the LISTA network.

%A similar unrolling process can be applied to Denoising-based Vector AMP (DVAMP) \cite{DVAMP} to form Learned DVAMP (LDVAMP). DVAMP is a variant of D-AMP that functions with a broader class of measurement matrices.











==> Learned D-AMP NIPS 2017_arxiv/Tables.tex <==
%Noise Free Experiments

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{PSNR of $128 \times 128$ reconstructions with i.i.d. Gaussian measurements and no measurement noise.}
    \begin{tabular}{r|rrrrrrr}
    \toprule
    \textbf{5\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 19.32 & 21.05 & 16.49 & 21.98 & 19.36 & 21.09 & 19.22 \\
    BM3D-AMP & 18.04 & 18.92 & 12.25 & 20.79 & 18.28 & 20.38 & 16.77 \\
    LDIT & 17.20 & 19.37 & 16.94 & 20.43 & 17.49 & 19.51 & 18.08 \\
    LDAMP & \textbf{21.26} & \textbf{22.44} & \textbf{17.04} & \textbf{22.84} & \textbf{21.30} & \textbf{22.74} & \textbf{20.17} \\
    NLR-CS & 20.31 & 21.51 & 14.96 & 22.05 & 19.69 & 21.55 & 19.22 \\
    \toprule
    \textbf{10\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 21.75 & 22.95 & 16.77 & 23.21 & 21.98 & 23.07 & 20.86 \\
    BM3D-AMP & 24.36 & 24.04 & \textbf{18.07} & 24.12 & 24.44 & 24.79 & 22.05 \\
    LDIT & 19.39 & 21.49 & 17.23 & 22.17 & 19.13 & 21.24 & 19.82 \\
    LDAMP & \textbf{25.80} & \textbf{24.67} & 17.36 & \textbf{24.37} & \textbf{26.00} & \textbf{25.43} & \textbf{22.52} \\
    NLR-CS & 25.17 & 23.84 & 17.84 & 23.56 & 25.18 & 24.91 & 21.80 \\
    \toprule
    \textbf{15\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 23.47 & 24.25 & 16.97 & 24.09 & 24.18 & 24.74 & 22.00 \\
    BM3D-AMP & 27.35 & 25.67 & 19.94 & 25.02 & 27.37 & 26.96 & 23.35 \\
    LDIT & 20.53 & 22.54 & 17.29 & 23.17 & 19.74 & 21.89 & 19.50 \\
    LDAMP & \textbf{28.78} & \textbf{26.79} & 17.65 & \textbf{25.40} & \textbf{29.38} & \textbf{27.65} & \textbf{23.97} \\
    NLR-CS & 28.10 & 25.57 & \textbf{20.11} & 24.45 & 28.06 & 26.82 & 23.10 \\
    \toprule
    \textbf{20\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 25.20 & 25.47 & 17.32 & 24.84 & 25.90 & 26.17 & 23.08 \\
    BM3D-AMP & 29.57 & 27.40 & {21.19} & 25.80 & 29.55 & 28.55 & 24.45 \\
    LDIT & 20.42 & 22.50 & 17.34 & 22.66 & 21.45 & 22.29 & 20.95 \\
    LDAMP & \textbf{31.10} & \textbf{28.58} & 18.07 & \textbf{26.31} & \textbf{31.88} & \textbf{29.57} & \textbf{25.21} \\
    NLR-CS & {30.42} & {27.34} & \textbf{21.29} & 25.56 & 30.47 & 28.54 & 24.18 \\
    \toprule
    \textbf{25\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 26.57 & 26.53 & 17.62 & 25.46 & 27.49 & 27.44 & 23.98 \\
    BM3D-AMP & 31.39 & 28.89 & 21.97 & 26.50 & 31.27 & 30.01 & 25.37 \\
    LDIT & 21.59 & 23.02 & 17.57 & 23.61 & 21.65 & 23.22 & 21.04 \\
    LDAMP & \textbf{32.68} & \textbf{30.17} & 18.13 & \textbf{27.06} & \textbf{33.87} & \textbf{31.06} & \textbf{26.20} \\
    NLR-CS & 32.42 & 28.78 & \textbf{22.04} & 26.52 & 32.47 & 30.13 & 25.26 \\
    \bottomrule
    \end{tabular}%
  \label{tab:GaussianPSNR}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Runtimes (seconds) of $128 \times 128$ reconstructions with i.i.d. Gaussian measurements and no measurement noise.}
    \begin{tabular}{l|rrrrr}
    \toprule
    \textbf{Sampling Rate} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{25\%} \\
    \midrule
    TVAL3 & 1.36  & 2.24  & 2.87  & 3.58  & 4.33 \\
    BM3D-AMP & 3.85  & 4.80  & 4.45  & 4.24  & 4.10 \\
    %BM3D-VAMP & 4.36  & 4.96  & 4.37  & 4.17  & 3.91 \\
    LDIT & 0.21  & 0.28  & 0.36  & 0.42  & 0.48 \\
    LDAMP & 0.34  & 0.40  & 0.49  & 0.55  & 0.61 \\
    %Learned D-VAMP & 0.34  & 0.38  & 0.51  & 0.55  & 0.64 \\
    NLR-CS & 67.83 & 85.91 & 103.87 & 124.35 & 146.29 \\
    \bottomrule
    \end{tabular}%
  \label{tab:GaussianTime}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
    \caption{PSNR of $128 \times 128$ reconstructions with coded diffraction measurements and no measurement noise.}
        \begin{tabular}{l|rrrrrrr}
        \toprule
    \textbf{5\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 21.66 & 22.70 & 16.79 & 23.20 & 21.94 & 22.98 & 20.92 \\
    BM3D-AMP & 18.37 & 17.89 & 13.46 & 13.32 & 17.80 & 16.91 & 20.83 \\
    LDIT & 20.20 & 21.09 & 16.69 & 22.31 & 19.07 & 20.85 & 19.98 \\
    LDAMP & \textbf{22.10} & \textbf{23.45} & \textbf{17.33} & \textbf{23.54} & \textbf{22.32} & \textbf{23.50} & \textbf{20.94} \\
    NLR-CS & 15.14 & 13.44 & 11.73 & 18.43 & 17.23 & 17.70 & 16.04 \\
    \toprule
    \textbf{10\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 25.08 & 25.39 & 17.34 & 24.79 & 25.83 & 26.13 & 23.13 \\
    BM3D-AMP & 25.40 & 24.48 & \textbf{18.68} & 24.48 & 25.52 & 25.53 & 22.56 \\
    LDIT & 24.02 & 24.77 & 17.31 & 24.74 & 24.36 & 25.24 & 20.21 \\
    LDAMP & \textbf{27.90} & \textbf{26.50} & 17.56 & \textbf{25.57} & \textbf{28.18} & \textbf{27.24} & \textbf{23.87} \\
    NLR-CS & 24.12 & 21.56 & 17.11 & 21.15 & 24.05 & 22.27 & 21.04 \\
    \toprule
    \textbf{15\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 27.78 & 27.71 & 17.96 & 26.05 & 28.90 & 28.54 & 24.90 \\
    BM3D-AMP & 28.96 & 25.98 & \textbf{20.39} & 25.12 & 28.67 & 27.11 & 23.63 \\
    LDIT & 28.44 & 26.59 & 17.31 & 25.73 & 30.21 & 26.92 & 24.28 \\
    LDAMP & \textbf{30.85} & \textbf{28.79} & 17.86 & \textbf{26.68} & \textbf{32.07} & \textbf{29.54} & \textbf{25.69} \\
    NLR-CS & 27.35 & 24.16 & 18.99 & 23.28 & 21.24 & 24.23 & 20.58 \\
    \toprule
    \textbf{20\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 30.05 & 29.93 & 18.73 & 27.32 & 31.62 & 30.77 & 26.55 \\
    BM3D-AMP & 32.08 & 28.07 & \textbf{21.41} & 25.89 & 31.47 & 28.99 & 24.57 \\
    LDIT & 31.60 & 28.61 & 17.30 & 26.06 & 32.15 & 30.49 & 25.57 \\
    LDAMP & \textbf{33.10} & \textbf{30.20} & 17.94 & \textbf{27.59} & \textbf{34.06} & \textbf{32.17} & \textbf{27.24} \\
    NLR-CS & 26.41 & 25.26 & 21.04 & 23.48 & 28.18 & 27.67 & 23.47 \\
    \toprule
    \textbf{25\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 32.37 & 32.13 & 19.63 & 28.63 & 34.20 & 33.05 & 28.12 \\
    BM3D-AMP & \textbf{34.69} & 29.59 & \textbf{22.26} & 26.36 & 34.74 & 30.51 & 25.69 \\
    LDIT & 34.00 & 30.43 & 17.65 & 26.24 & 35.37 & 31.02 & 27.63 \\
    LDAMP & 34.58 & \textbf{32.62} & 18.60 & \textbf{29.01} & \textbf{36.07} & \textbf{33.86} & \textbf{28.60} \\
    NLR-CS & 31.74 & 28.16 & 20.64 & 25.79 & 28.60 & 28.89 & 21.04 \\
    \bottomrule
    \end{tabular}%
  \label{tab:CodedDiffractionPSNR}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Runtimes (seconds) of $128 \times 128$ reconstructions with coded diffraction measurements and no measurement noise.}
    \begin{tabular}{l|rrrrr}
    \toprule
    \textbf{Sampling Rate} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{25\%} \\
    \midrule
    TVAL3 & 0.62  & 0.52  & 0.46  & 0.43  & 0.41 \\
    BM3D-AMP & 3.80  & 4.55  & 4.29  & 3.67  & 3.40 \\
    %BM3D-VAMP & 3.86  & 4.47  & 3.47  & 2.85  & 2.41 \\
    LDIT & 0.13  & 0.14  & 0.14  & 0.14  & 0.14 \\
    LDAMP & 0.26  & 0.26  & 0.26  & 0.27  & 0.26 \\
    %Learned D-VAMP & 0.27  & 0.26  & 0.27  & 0.29  & 0.27 \\
    NLR-CS & 87.26 & 87.82 & 87.43 & 87.18 & 86.87 \\
    \bottomrule
    \end{tabular}%
  \label{tab:CodedDiffractionTime}%
\end{table}%


%%Noisy Experiments


\begin{table*}[t]
  \centering
  \caption{PSNR of reconstruction of $128 \times 128$ Boat test image with additive white Gaussian measurement noise (AWGN) with various standard deviations  (s.d.).}
    \begin{tabular}{r|rrrrr}
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 10}} \\
    \midrule
    \textbf{Sampling rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 21.08 & 22.84 & 24.06 & 24.97 & 25.75 \\
    BM3D-AMP & 16.99 & 23.98 & 25.40 & 26.79 & 27.64 \\
    LDAMP & 22.41 & 24.56 & 26.36 & 27.62 & 28.56 \\
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 20}} \\
    \midrule
    \textbf{Sampling Rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 21.00 & 22.60 & 23.50 & 23.94 & 24.16 \\
    BM3D-AMP & 21.03 & 23.67 & 24.63 & 25.45 & 26.03 \\
    LDAMP & 22.33 & 24.24 & 25.35 & 26.33 & 26.75 \\
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 30}} \\
    \midrule
    \textbf{Sampling Rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 20.90 & 22.23 & 22.74 & 22.74 & 22.57 \\
    BM3D-AMP & 18.43 & 23.34 & 24.09 & 24.46 & 24.80 \\
    LDAMP & 22.11 & 23.80 & 24.55 & 25.10 & 25.34 \\
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 40}} \\
    \midrule
    \textbf{Sampling Rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 20.77 & 21.80 & 21.93 & 21.60 & 21.12 \\
    BM3D-AMP & 19.24 & 23.02 & 23.55 & 23.77 & 23.94 \\
    LDAMP & 21.85 & 23.41 & 23.90 & 24.33 & 24.50 \\
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 50}} \\
    \midrule
    \textbf{Sampling Rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 20.58 & 21.33 & 21.17 & 20.53 & 19.84 \\
    BM3D-AMP & 19.45 & 22.69 & 23.13 & 23.28 & 23.38 \\
    LDAMP & 21.58 & 22.96 & 23.44 & 23.65 & 23.76 \\
    \toprule
    \end{tabular}%
  \label{tab:NoisyPerformance}%
\end{table*}%


==> Learned D-AMP NIPS 2017_arxiv/TheoreticalAnalysis.tex <==
\section{Theoretical analysis of LDAMP}

This section makes two theoretical contributions. First, we show that the state-evolution (S.E.), a framework that predicts the performance of AMP/D-AMP, holds for LDAMP as well.\footnote{For D-AMP and LDAMP, the S.E.~is entirely observational; no rigorous theory exists. For AMP, the S.E.~has been proven asymptotically accurate for i.i.d.~Gaussian measurements \cite{bayati2011dynamics}.} Second, we use the S.E.~to prove that layer-by-layer and denoiser-by-denoiser training of LDAMP are MMSE optimal.

\subsection{State-evolution}\label{ssec:SE}

%The AMP/D-AMP S.E.~is a series of equations that predicts the performance of the algorithm over each of its iterations \cite{DoMaMo09, bayati2011dynamics, DAMPITIT}.\footnote{For D-AMP (and LDAMP), the S.E.~is entirely observational; no rigorous theory exists. For AMP, the S.E.~has been proven asymptotically accurate with i.i.d.~Gaussian measurements \cite{bayati2011dynamics}.} 
In the context of LAMP and LDAMP, the S.E.~equations predict the intermediate mean squared error (MSE) of the network over each of its layers \cite{LAMP}. %In this section we review the S.E.~and present our main theoretical finding; the S.E.~holds for LDAMP.
% Note that the S.E.~we provide here is the ``deterministic'' state-evolution proposed in \cite{DAMPITIT} to predict the performance of D-AMP. This state-evolution is distinct from the widely studied ``probabilistic'' state-evolution proposed in \cite{DoMaMo09}, proven, for some contexts, in \cite{bayati2011dynamics}, and verified for LAMP and LVAMP in \cite{LAMP}. The ``deterministic'' S.E.~fixes the signal $x_o$ and takes the expectation over the distribution of the noise. By contrast, the ``probabilistic'' S.E.~takes the expectation over the distribution of both the signal and the noise.
Starting from $\theta^0 = \frac{\|x_o\|_2^2}{n}$ the S.E.~generates a sequence of numbers through the following iterations:
\begin{equation}\label{eq:stateevo1}
\theta^{l+1}(x_o, \delta, \sigma_\epsilon^2) = \frac{1}{n}  \mathbb{E}_\epsilon \| D^l_{w^l(\sigma)} (x_o + \sigma^l \epsilon) -x_o \|_2^2, 
\end{equation}
where $(\sigma^l)^2 = \frac{1}{\delta}\theta^l(x_o, \delta, \sigma_\epsilon^2) + \sigma_\epsilon^2$, the scalar $\sigma_\epsilon$ is the standard deviation of the measurement noise $\epsilon$, and the expectation is with respect to $\epsilon \sim N(0,I)$.
Note that the notation $\theta^{l+1}(x_o, \delta, \sigma_\epsilon^2)$ is used to emphasize that $\theta^l$ may depend on the signal $x_o$, the under-determinacy $\delta$, and the measurement noise. 

Let $x^l$ denote the estimate at layer $l$ of LDAMP. Our empirical findings, illustrated in Figure \ref{fig:StateEvolution}, show that the MSE of LDAMP is predicted accurately by the S.E. We formally state our finding.

\begin{figure}[t]
 \begin{center}
 	%\begin{center}
 	% Requires \usepackage{graphicx} 
 	%\vspace{-1cm}
 	\includegraphics[width=.70\textwidth]{./figs/SEplot_10percent_128boat_nonoise.png} 
 	%\vspace{-1.5cm}
 	\caption{The MSE of intermediate reconstructions of the Boat test image across different layers for the DnCNN variants of LDAMP and LDIT alongside their predicted S.E. The image was sampled with Gaussian measurements at a rate of $\frac{m}{n}=0.1$. Note that LDAMP is well predicted by the S.E., whereas LDIT is not.}
 	\label{fig:StateEvolution} 
 \end{center}
\end{figure}

\begin{finding}\label{find:mainone}
If the LDAMP network starts from $x^0=0$, then for large values of $m$ and $n$, the S.E.~predicts the mean square error of LDAMP at each layer, i.e., 
$
\theta^l (x_o, \delta, \sigma_\epsilon^2) \approx \frac{1}{n} \left\|x^l-x_o \right\|_2^2, 
$
if the following conditions hold:
(i) The elements of the matrix $\mathbf{A}$ are i.i.d.\ Gaussian (or subgaussian) with mean zero and standard deviation $1/m$. %\footnote{The LDVAMP S.E.~likely holds over a broader class of matrices, however this has not been confirmed.}
(ii) The noise $w$ is also i.i.d.\ Gaussian. 
(iii) The denoisers $D^l$ at each layer are Lipschitz continuous.\footnote{A denoiser is said to be $L$-Lipschitz continuous if for every $x_1,x_2 \in C$ we have $\|D(x_1)-D(x_2)\|_2^2\leq L \|x_1-x_2\|_2^2.$ While we did not find it necessary in practice, weight clipping and gradient norm penalization can be used to ensure Lipschitz continuity of the convolutional denoiser \cite{gulrajani2017improved}.}
\end{finding}

%Figure \ref{fig:StateEvolution} demonstrates the accuracy of the state-evolution predictions under the proposed conditions.

%The S.E.~is a flexible tool to prove properties about D-AMP. For instance, it has been used to determine under what conditions D-AMP will recover a signal, how accurately D-AMP will recover a signal in the presence of noise, and how one should tune D-AMP \cite{DAMPITIT}. In this work we use the S.E.~to prove that layer-by-layer and denoiser-by-denoiser training of LDAMP is minimum mean squared error (MMSE) optimal.

\subsection{Layer-by-layer and denoiser-by-denoiser training is optimal}\label{ssec:trainingtheory}

%The central challenge to using LDAMP in practice is training; that is learning the network's many free parameters. An $L$ layer LDAMP network consists of $L$ denoisers $D^1,D^2,...D^L$, each with their own sets of weights/parameters $w^1, w^2, ...w^L$. Together they parameterize the LDAMP network with $w=[w^1,w^2,...w^L]$. In this work we test a ten layer network that uses the DnCNN denoiser at each layer. Each DnCNN denoiser is parameterized by roughly 600000 parameters. As a result, the 10 layer DnCNN-based  network has over 6 {\em million} parameters to train; $w\in\mathbb{R}^{6000000}$. Naively training such a large network is a computationally brutal task. Fortunately, the state-evolution framework allows us to prove the following powerful result: Layer-by-layer training of is MMSE optimal. We state the result formally.

The S.E.~framework enables us to prove the following results: Layer-by-layer and denoiser-by-denoiser training of LDAMP are MMSE optimal. %; they minimize $\mathbb{E}\|x^L-x_o\|^2$. 
Both these results rely upon the following lemma.%, which states that layer-by-layer training minimizes the expectation of the state evolution predictions.

\begin{lemma}\label{lem:GreedyParams}
Suppose that $D^1,D^2,... D^L$ are monotone denoisers in the sense that for $l=1,2,...L$ $\inf_{w^l} \mathbb{E} \|D^l_{w^l(\sigma)} (x_o + \sigma \epsilon) -x_o \|_2^2$ is a non-decreasing function of $\sigma$. %\footnote{In layman's terms, this implies that adding noise to the denoiser's input will not increase the accuracy of the denoiser's output.}
If the weights $w^1$ of $D^1$ are set to minimize $\mathbb{E}_{x_0}[\theta^1]$ and fixed; and then the weights $w^2$ of $D^2$ are set to minimize $\mathbb{E}_{x_0}[\theta^2]$ and fixed, \dots and then the weights $w^L$ of $D^L$ are set to minimize $\mathbb{E}_{x_0}[\theta^L]$, then together they minimize $\mathbb{E}_{x_0}[\theta^L]$.
%If $D^1$ is trained to minimize $\frac{1}{n}\|x^1-x_o\|_2^2$, and then $D^1$ is trained to minimize $\frac{1}{n}\|x^L-x_o\|_2^2$, ... and then $D^L$ is trained to minimize $\frac{1}{n}\|x^L-x_o\|_2^2$ then together they minimize $\frac{1}{n}\|x^L-x_o\|_2^2$.
%, D^2, ... D^L$ are trained independently to minimize $\frac{1}{n}\|x^1-x_o\|_2^2, \frac{1}{n}\|x^1-x_o\|_2^2, ... \frac{1}{n}\|x^L-x_o\|_2^2$, respectively, then together they also minimize $\theta^L$.
%If $D^1, D^2, ... D^L$ are trained to minimize $\theta^1, \theta^2, ... \theta^L$, respectively, then together they also minimize $\theta^L$.
\end{lemma}

Lemma \ref{lem:GreedyParams} can be derived using the proof technique for Lemma 3 of \cite{DAMPITIT}, but with $\theta_l$ replaced by $\mathbb{E}_{x_0} [\theta^l]$ throughout. It leads to the following two results.

%One challenge in applying the above result to our work is that we are not interested in training the weights to minimize the reconstruction error with a single $x_o$ but rather the reconstruction error for all $x_o\in \mathcal{C}$. That is, we are not interested in minimizing $\theta^L$ but rather $\mathbb{E}_{x_0}[\theta^L]$.

\begin{corollary}\label{cor:LbyLtraining}
Under the conditions in Lemma \ref{lem:GreedyParams}, layer-by-layer training of LDAMP is MMSE optimal.
\end{corollary}

This result follows from Lemma \ref{lem:GreedyParams} and the equivalence between $\mathbb{E}_{x_0}[\theta^l]$ and $\mathbb{E}_{x_0}[\frac{1}{n}\|x^l-x_o\|_2^2]$.

\begin{corollary}\label{cor:DbyDtraining}
Under the conditions in Lemma \ref{lem:GreedyParams}, denoiser-by-denoiser training of LDAMP is MMSE optimal.
\end{corollary}

This result follows from Lemma \ref{lem:GreedyParams} and the equivalence between $\mathbb{E}_{x_0}[\theta^l]$ and $\mathbb{E}_{x_0}[\frac{1}{n}  \mathbb{E}_\epsilon \| D^l_{w^l(\sigma)} (x_o + \sigma^l \epsilon) -x_o \|_2^2]$.









%\textcolor{red}{This probably needs a little more information.}


%\subsection{Resources allocation}
%S.E.~ tells us if it is better to train a weak denoiser for many iterations or a strong denoiser for a few.

% \subsection{Computational Complexity}

% In this section we demonstrate that in the high dimensional setting LDAMP with the DnCNN denoiser is computationally efficient.

% % In this section we prove that  is nearly as fast as the fastest possible recovery algorithm. To do so, we first prove the following lemma.

% % \textcolor{red}{Issue with proof: We could simply toss out $m-k$ of the measurements and reconstruct the signal.}

% % \begin{lemma}
% % Given a dense $m\times n$ measurement matrix $\mathbf{A}$ with i.i.d. Gaussian distributed elements, a $k$ sparse signal $x$, and measurements of the form $y=\mathbf{A}x$, any compressive sensing recovery algorithm will require at least $nk$ multiply operations to recover $x$.
% % \begin{proof}
% % Consider a simple problem.
% % \begin{align}\label{eqn:linear}
% % \text{Find }x\text{ such that }\|y-\mathbf{A}x\|\leq \epsilon.
% % \end{align}
% % If $\|y\|\geq\epsilon$ this requires $mn$ operations.\cite{}. Any algorithm that can solve the CS synthesis problem \eqref{eqn:CS_synthesis} can necessarily solve \eqref{eqn:linear}:  \eqref{eqn:linear} is just the measurement constraint from \eqref{eqn:CS_synthesis}. Thus $O(mn)$ lower bounds the computational complexity of solving the CS problem \eqref{eqn:CS_synthesis}.
% % \end{proof}
% % \end{lemma}

% \begin{lemma}
% Given a dense $m\times n$ measurement matrix $\mathbf{A}$ with i.i.d. Gaussian distributed elements, in the high dimensional setting LDAMP with $L$ layers and the DnCNN denoiser is no more than $2L+1$ times slower than any other recovery algorithm that performs a matrix multiply with $\mathbf{A}$.
% \begin{proof}
% The computational complexity of the DnCNN version of LDAMP is dominated by $2L$ matrix multiplies and $2L$ denoiser operations.
% Each DnCNN denoiser convolves $\sqrt{n}\times \sqrt{n} \times 64$ feature maps with $3\times 3 \times 64$ filters, which has a computational complexity $O(n\log n)$. 
% Each matrix multiply has a computational complexity of $O(mn)$.
% Thus the computational complexity of the DnCNN version of LDAMP is $O(2Lmn+Ln\log n)$. 
% With $m>\log n$, for large $m$ and $n$ the computational complexity of the DnCNN version of LDAMP is less than $O((2L+1)mn)$.
% \end{proof}
% \end{lemma}


==> Learned D-AMP NIPS 2017_arxiv/Training.tex <==
\section{Training the LDIT and LDAMP networks}\label{sec:Training}

We experimented with three different methods to train the LDIT and LDAMP networks. Here we describe and compare these training methods at a high level; the details are described in Section \ref{sec:expmt}. 
\begin{itemize}
    \item {\bf End-to-end training:} We train all the weights of the network simultaneously. This is the standard method of training a neural network.
    \item {\bf Layer-by-layer training:} We train a 1 AMP layer network (which itself contains a 16-20 layer denoiser) to recover the signal, fix these weights, add an AMP layer, train the second layer of the resulting 2 layer network to recover the signal, fix these weights, and repeat until we have trained a 10 layer network.% We found training a network layer-by-layer made it far less senstitive to initialization, as compared to an end-to-end trained network.
    \item {\bf Denoiser-by-denoiser training:} We decouple the denoisers from the rest of the network and train each on AWGN denoising problems at different noise levels. During inference, the network uses its estimate of the standard deviation of the noise to select which set of denoiser weights to use. Note that, in selecting which denoiser weights to use, we must discretize the expected range of noise levels; e.g., if $\hat{\sigma}=35$, then we use the denoiser for noise standard deviations between $20$ and $40$.
\end{itemize}

% \paragraph{Layer-by-layer training}
% We trained the network layer-by-layer by optimizing the first layer's weights, fixing these weights, and then optimizing the next layer, etc. 
% Resulting network becomes specific to certain sampling rates, signal dimensions, and noise levels and does not generalize to new problems. Moreover, because training each layer required feeding data through all the previous layers, this method was relatively slow to train.

% \paragraph{End-to-end training}
% We trained the network end-to-end by feeding in training data through the entire network and updating all of the weights simultaneously. As in layer-by-layer training, such a network does not generalize to new problems. In addition, because this method feeds data through many layers and updates parameters at each of these layers the network is slow to train. To speed training and avoid exploding gradients, we initialized the weights of the end-to-end network using results from layer-by-layer training. When training LDAMP end-to-end we did not propagate gradients through the Monte-Carlo estimate of the divergence.

% \paragraph{Denoiser-by-denoiser training}
% We trained ten denoisers independently by decoupling the denoisers from the rest of the network and training each on AWGN denoising problems at different noise levels. During inference the network used its estimate of the standard deviation of the noise to select which set of denoiser weights to use. Note that this method automatically generalizes to new sampling rates and problem dimensions; by using weights based on the estimate of the standard deviation of the effective noise the network is able to automatically adapt to different setups.

%\vspace{-4 mm}
\paragraph{Comparing Training Methods.}
Stochastic gradient descent theory suggests that layer-by-layer and denoiser-by-denoiser training should sacrifice performance as compared to end-to-end training \cite{smieja1993neural}. In Section \ref{ssec:trainingtheory} we will prove that this is not the case for LDAMP. {\em For LDAMP, layer-by-layer and denoiser-by-denoiser training are minimum-mean-squared-error (MMSE) optimal}. %These results have major practical implications. Layer-by-layer training and denoiser-by-denoiser training is is more stable and significantly faster than end-to-end training. %: XXX seconds and XXX seconds, respectively, versus XXXX seconds for end-to-end training.
%More importantly, a network trained in a denoiser-by-denoiser fashion is far more generalizable; it can handle different samping rates, noise levels, etc.. 
These theoretical results are born out experimentally in Tables \ref{tab:TrainingComparo2020} and \ref{tab:TrainingComparo2005}. Each of the networks tested in this section consists of 10 unrolled DAMP/DIT layers that each contain a 16 layer DnCNN denoiser.



\newcommand{\mytabone}{% Just for this example
  \begin{tabular}{lcc}
  \toprule
          & \multicolumn{1}{l}{LDIT} & \multicolumn{1}{l}{LDAMP} \\
    End-to-end & 32.1  & 33.1 \\
    Layer-by-layer & 26.1  & 33.1 \\
    Denoiser-by-denoiser & 28.0  & 31.6 \\
    \bottomrule
    \end{tabular}%
    \label{tab:TrainingComparo2020}%
}

\newcommand{\mytabtwo}{% Just for this example
  \begin{tabular}{lcc}
  \toprule
          & \multicolumn{1}{l}{LDIT} & \multicolumn{1}{l}{LDAMP} \\
    End-to-end & 8.0   & 18.7 \\
    Layer-by-layer & -2.6  & 18.7 \\
    Denoiser-by-denoiser & 22.1  & 25.9 \\
    \bottomrule
    \end{tabular}%
    \label{tab:TrainingComparo2005}
}



\begin{figure}%
  \centering
  \subfigure[][]{\mytabone}%
  \qquad
  \subfigure[][]{\mytabtwo}
  \caption{Average PSNRs\protect\footnotemark~of 100 $40 \times 40$ image reconstructions with i.i.d.~Gaussian measurements trained at a sampling rate of $\frac{m}{n}=0.20$ and tested at sampling rates of $\frac{m}{n}=0.20$ (a) and $\frac{m}{n}=0.05$ (b).}%
  %\caption{Average PSNRs~of 100 $40 \times 40$ image reconstructions with i.i.d.~Gaussian measurements trained at a sampling rate of $\frac{m}{n}=0.20$ and tested at sampling rates of $\frac{m}{n}=0.20$ (a) and $\frac{m}{n}=0.05$ (b).}%
  \label{fig:table}%
\end{figure}
\footnotetext{${\rm PSNR} = 10 \log_{10}(\frac{255^2}{{\rm mean}((\hat{x}-x_o)^2)})$ when the pixel range is 0 to 255.}


% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[t]
%   \centering
%   \caption{Average PSNR\footnotemark of 100 $40 \times 40$ image reconstructions with i.i.d.~Gaussian measurements trained at a sampling rate of $\frac{m}{n}=0.20$ and tested at a sampling rate of $\frac{m}{n}=0.20$.}
%         \begin{tabular}{lccc}
%         \toprule
%           & End-to-end & Layer-by-layer & Denoiser-by-denoiser \\
%     LDIT  & 32.1  & 26.1  & 28.0 \\
%     LDAMP & 33.1  & 33.1  & 31.6 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:TrainingComparo2020}%
% \end{table}%
% \footnotetext{${\rm PSNR} = 10 \log_{10}(\frac{255^2}{{\rm mean}((\hat{x}-x_o)^2)})$ when the pixel range is 0 to 255.}



Table \ref{tab:TrainingComparo2020} demonstrates that, as suggested by theory, layer-by-layer training of LDAMP is optimal; additional end-to-end training does not improve the performance of the network. 
In contrast, the table demonstrates that layer-by-layer training of LDIT, which represents the behavior of a typical neural network, is suboptimal; additional end-to-end training dramatically improves its performance. 

Despite the theoretical result the denoiser-by-denoiser training is optimal, Table \ref{tab:TrainingComparo2020} shows that LDAMP trained denoiser-by-denoiser performs slightly worse than the end-to-end and layer-by-layer trained networks. This gap in performance is likely due to the discretization of the noise levels, which is not modeled in our theory. This gap can be reduced by using a finer discretization of the noise levels or by using deeper denoiser networks that can better handle a range of noise levels \cite{DnCNN}. %In Section \ref{sec:expmt} we use deeper denoiser networks.


% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[t]
%   \centering
%   \caption{Average PSNR of 100 $40 \times 40$ reconstructions with i.i.d.~Gaussian measurements trained at a sampling rate of $\frac{m}{n}=0.20$ and tested at a sampling rate of $\frac{m}{n}=0.05$.}
%     \begin{tabular}{lccc}
%           \toprule
%           & End-to-end & Layer-by-layer & Denoiser-by-denoiser \\
%     LDIT  & 8.0   & -2.6  & 22.1 \\
%     LDAMP & 18.7  & 18.7  & 25.9 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:TrainingComparo2005}%
% \end{table}%




In Table \ref{tab:TrainingComparo2005} we report on the performance of the two networks when trained at a one sampling rate and tested at another.
LDIT and LDAMP networks trained end-to-end and layer-by-layer at a sampling rate of $\frac{m}{n}=0.2$ perform poorly when tested at a sampling rate of $\frac{m}{n}=0.05$.
In contrast, the denoiser-by-denoiser trained networks, which were not trained at a specific sampling rate, generalize well to different sampling rates.


==> Tables.tex <==
%Noise Free Experiments

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{PSNR of $128 \times 128$ reconstructions with i.i.d. Gaussian measurements and no measurement noise.}
    \begin{tabular}{r|rrrrrrr}
    \toprule
    \textbf{5\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 19.32 & 21.05 & 16.49 & 21.98 & 19.36 & 21.09 & 19.22 \\
    BM3D-AMP & 18.04 & 18.92 & 12.25 & 20.79 & 18.28 & 20.38 & 16.77 \\
    LDIT & 17.20 & 19.37 & 16.94 & 20.43 & 17.49 & 19.51 & 18.08 \\
    LDAMP & \textbf{21.26} & \textbf{22.44} & \textbf{17.04} & \textbf{22.84} & \textbf{21.30} & \textbf{22.74} & \textbf{20.17} \\
    NLR-CS & 20.31 & 21.51 & 14.96 & 22.05 & 19.69 & 21.55 & 19.22 \\
    \toprule
    \textbf{10\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 21.75 & 22.95 & 16.77 & 23.21 & 21.98 & 23.07 & 20.86 \\
    BM3D-AMP & 24.36 & 24.04 & \textbf{18.07} & 24.12 & 24.44 & 24.79 & 22.05 \\
    LDIT & 19.39 & 21.49 & 17.23 & 22.17 & 19.13 & 21.24 & 19.82 \\
    LDAMP & \textbf{25.80} & \textbf{24.67} & 17.36 & \textbf{24.37} & \textbf{26.00} & \textbf{25.43} & \textbf{22.52} \\
    NLR-CS & 25.17 & 23.84 & 17.84 & 23.56 & 25.18 & 24.91 & 21.80 \\
    \toprule
    \textbf{15\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 23.47 & 24.25 & 16.97 & 24.09 & 24.18 & 24.74 & 22.00 \\
    BM3D-AMP & 27.35 & 25.67 & 19.94 & 25.02 & 27.37 & 26.96 & 23.35 \\
    LDIT & 20.53 & 22.54 & 17.29 & 23.17 & 19.74 & 21.89 & 19.50 \\
    LDAMP & \textbf{28.78} & \textbf{26.79} & 17.65 & \textbf{25.40} & \textbf{29.38} & \textbf{27.65} & \textbf{23.97} \\
    NLR-CS & 28.10 & 25.57 & \textbf{20.11} & 24.45 & 28.06 & 26.82 & 23.10 \\
    \toprule
    \textbf{20\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 25.20 & 25.47 & 17.32 & 24.84 & 25.90 & 26.17 & 23.08 \\
    BM3D-AMP & 29.57 & 27.40 & {21.19} & 25.80 & 29.55 & 28.55 & 24.45 \\
    LDIT & 20.42 & 22.50 & 17.34 & 22.66 & 21.45 & 22.29 & 20.95 \\
    LDAMP & \textbf{31.10} & \textbf{28.58} & 18.07 & \textbf{26.31} & \textbf{31.88} & \textbf{29.57} & \textbf{25.21} \\
    NLR-CS & {30.42} & {27.34} & \textbf{21.29} & 25.56 & 30.47 & 28.54 & 24.18 \\
    \toprule
    \textbf{25\% Sampling} & \textbf{Barbara} & \textbf{Boat} & \textbf{Fingerprint} & \textbf{Mandrill} & \textbf{Peppers} & \textbf{Couple} & \textbf{Stream \& Bridge} \\
    \midrule
    TVAL3 & 26.57 & 26.53 & 17.62 & 25.46 & 27.49 & 27.44 & 23.98 \\
    BM3D-AMP & 31.39 & 28.89 & 21.97 & 26.50 & 31.27 & 30.01 & 25.37 \\
    LDIT & 21.59 & 23.02 & 17.57 & 23.61 & 21.65 & 23.22 & 21.04 \\
    LDAMP & \textbf{32.68} & \textbf{30.17} & 18.13 & \textbf{27.06} & \textbf{33.87} & \textbf{31.06} & \textbf{26.20} \\
    NLR-CS & 32.42 & 28.78 & \textbf{22.04} & 26.52 & 32.47 & 30.13 & 25.26 \\
    \bottomrule
    \end{tabular}%
  \label{tab:GaussianPSNR}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Runtimes (seconds) of $128 \times 128$ reconstructions with i.i.d. Gaussian measurements and no measurement noise.}
    \begin{tabular}{l|rrrrr}
    \toprule
    \textbf{Sampling Rate} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{25\%} \\
    \midrule
    TVAL3 & 1.36  & 2.24  & 2.87  & 3.58  & 4.33 \\
    BM3D-AMP & 3.85  & 4.80  & 4.45  & 4.24  & 4.10 \\
    %BM3D-VAMP & 4.36  & 4.96  & 4.37  & 4.17  & 3.91 \\
    LDIT & 0.21  & 0.28  & 0.36  & 0.42  & 0.48 \\
    LDAMP & 0.34  & 0.40  & 0.49  & 0.55  & 0.61 \\
    %Learned D-VAMP & 0.34  & 0.38  & 0.51  & 0.55  & 0.64 \\
    NLR-CS & 67.83 & 85.91 & 103.87 & 124.35 & 146.29 \\
    \bottomrule
    \end{tabular}%
  \label{tab:GaussianTime}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
    \caption{PSNR of $128 \times 128$ reconstructions with coded diffraction measurements and no measurement noise.}
        \begin{tabular}{l|rrrrrrr}
        \toprule
    \textbf{5\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 21.66 & 22.70 & 16.79 & 23.20 & 21.94 & 22.98 & 20.92 \\
    BM3D-AMP & 18.37 & 17.89 & 13.46 & 13.32 & 17.80 & 16.91 & 20.83 \\
    LDIT & 20.20 & 21.09 & 16.69 & 22.31 & 19.07 & 20.85 & 19.98 \\
    LDAMP & \textbf{22.10} & \textbf{23.45} & \textbf{17.33} & \textbf{23.54} & \textbf{22.32} & \textbf{23.50} & \textbf{20.94} \\
    NLR-CS & 15.14 & 13.44 & 11.73 & 18.43 & 17.23 & 17.70 & 16.04 \\
    \toprule
    \textbf{10\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 25.08 & 25.39 & 17.34 & 24.79 & 25.83 & 26.13 & 23.13 \\
    BM3D-AMP & 25.40 & 24.48 & \textbf{18.68} & 24.48 & 25.52 & 25.53 & 22.56 \\
    LDIT & 24.02 & 24.77 & 17.31 & 24.74 & 24.36 & 25.24 & 20.21 \\
    LDAMP & \textbf{27.90} & \textbf{26.50} & 17.56 & \textbf{25.57} & \textbf{28.18} & \textbf{27.24} & \textbf{23.87} \\
    NLR-CS & 24.12 & 21.56 & 17.11 & 21.15 & 24.05 & 22.27 & 21.04 \\
    \toprule
    \textbf{15\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 27.78 & 27.71 & 17.96 & 26.05 & 28.90 & 28.54 & 24.90 \\
    BM3D-AMP & 28.96 & 25.98 & \textbf{20.39} & 25.12 & 28.67 & 27.11 & 23.63 \\
    LDIT & 28.44 & 26.59 & 17.31 & 25.73 & 30.21 & 26.92 & 24.28 \\
    LDAMP & \textbf{30.85} & \textbf{28.79} & 17.86 & \textbf{26.68} & \textbf{32.07} & \textbf{29.54} & \textbf{25.69} \\
    NLR-CS & 27.35 & 24.16 & 18.99 & 23.28 & 21.24 & 24.23 & 20.58 \\
    \toprule
    \textbf{20\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 30.05 & 29.93 & 18.73 & 27.32 & 31.62 & 30.77 & 26.55 \\
    BM3D-AMP & 32.08 & 28.07 & \textbf{21.41} & 25.89 & 31.47 & 28.99 & 24.57 \\
    LDIT & 31.60 & 28.61 & 17.30 & 26.06 & 32.15 & 30.49 & 25.57 \\
    LDAMP & \textbf{33.10} & \textbf{30.20} & 17.94 & \textbf{27.59} & \textbf{34.06} & \textbf{32.17} & \textbf{27.24} \\
    NLR-CS & 26.41 & 25.26 & 21.04 & 23.48 & 28.18 & 27.67 & 23.47 \\
    \toprule
    \textbf{25\% Sampling} & \multicolumn{1}{l}{\textbf{Barbara}} & \multicolumn{1}{l}{\textbf{Boat}} & \multicolumn{1}{l}{\textbf{Fingerprint}} & \multicolumn{1}{l}{\textbf{Mandrill}} & \multicolumn{1}{l}{\textbf{Peppers}} & \multicolumn{1}{l}{\textbf{Couple}} & \multicolumn{1}{l}{\textbf{Stream \& Bridge}} \\
    \midrule
    TVAL3 & 32.37 & 32.13 & 19.63 & 28.63 & 34.20 & 33.05 & 28.12 \\
    BM3D-AMP & \textbf{34.69} & 29.59 & \textbf{22.26} & 26.36 & 34.74 & 30.51 & 25.69 \\
    LDIT & 34.00 & 30.43 & 17.65 & 26.24 & 35.37 & 31.02 & 27.63 \\
    LDAMP & 34.58 & \textbf{32.62} & 18.60 & \textbf{29.01} & \textbf{36.07} & \textbf{33.86} & \textbf{28.60} \\
    NLR-CS & 31.74 & 28.16 & 20.64 & 25.79 & 28.60 & 28.89 & 21.04 \\
    \bottomrule
    \end{tabular}%
  \label{tab:CodedDiffractionPSNR}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Runtimes (seconds) of $128 \times 128$ reconstructions with coded diffraction measurements and no measurement noise.}
    \begin{tabular}{l|rrrrr}
    \toprule
    \textbf{Sampling Rate} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{25\%} \\
    \midrule
    TVAL3 & 0.62  & 0.52  & 0.46  & 0.43  & 0.41 \\
    BM3D-AMP & 3.80  & 4.55  & 4.29  & 3.67  & 3.40 \\
    %BM3D-VAMP & 3.86  & 4.47  & 3.47  & 2.85  & 2.41 \\
    LDIT & 0.13  & 0.14  & 0.14  & 0.14  & 0.14 \\
    LDAMP & 0.26  & 0.26  & 0.26  & 0.27  & 0.26 \\
    %Learned D-VAMP & 0.27  & 0.26  & 0.27  & 0.29  & 0.27 \\
    NLR-CS & 87.26 & 87.82 & 87.43 & 87.18 & 86.87 \\
    \bottomrule
    \end{tabular}%
  \label{tab:CodedDiffractionTime}%
\end{table}%


%%Noisy Experiments


\begin{table*}[t]
  \centering
  \caption{PSNR of reconstruction of $128 \times 128$ Boat test image with additive white Gaussian measurement noise (AWGN) with various standard deviations  (s.d.).}
    \begin{tabular}{r|rrrrr}
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 10}} \\
    \midrule
    \textbf{Sampling rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 21.08 & 22.84 & 24.06 & 24.97 & 25.75 \\
    BM3D-AMP & 16.99 & 23.98 & 25.40 & 26.79 & 27.64 \\
    LDAMP & 22.41 & 24.56 & 26.36 & 27.62 & 28.56 \\
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 20}} \\
    \midrule
    \textbf{Sampling Rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 21.00 & 22.60 & 23.50 & 23.94 & 24.16 \\
    BM3D-AMP & 21.03 & 23.67 & 24.63 & 25.45 & 26.03 \\
    LDAMP & 22.33 & 24.24 & 25.35 & 26.33 & 26.75 \\
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 30}} \\
    \midrule
    \textbf{Sampling Rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 20.90 & 22.23 & 22.74 & 22.74 & 22.57 \\
    BM3D-AMP & 18.43 & 23.34 & 24.09 & 24.46 & 24.80 \\
    LDAMP & 22.11 & 23.80 & 24.55 & 25.10 & 25.34 \\
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 40}} \\
    \midrule
    \textbf{Sampling Rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 20.77 & 21.80 & 21.93 & 21.60 & 21.12 \\
    BM3D-AMP & 19.24 & 23.02 & 23.55 & 23.77 & 23.94 \\
    LDAMP & 21.85 & 23.41 & 23.90 & 24.33 & 24.50 \\
    \toprule
    \multicolumn{6}{c}{\textbf{AWGN with s.d. 50}} \\
    \midrule
    \textbf{Sampling Rate (\%)} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} \\
    \midrule
    TVAL3 & 20.58 & 21.33 & 21.17 & 20.53 & 19.84 \\
    BM3D-AMP & 19.45 & 22.69 & 23.13 & 23.28 & 23.38 \\
    LDAMP & 21.58 & 22.96 & 23.44 & 23.65 & 23.76 \\
    \toprule
    \end{tabular}%
  \label{tab:NoisyPerformance}%
\end{table*}%

